Panoptic Neural Fields: A Semantic Object-Aware Neural Scene Representation

We present Panoptic Neural Fields (PNF), an object-aware neural scene representation that decomposes a scene into a set of objects (things) and background (stuff). Each object is represented by an oriented 3D bounding box and a multi-layer perceptron (MLP) that takes position, direction, and time and outputs density and radiance. The background stuff is represented by a similar MLP that additionally outputs semantic labels. Each object MLPs are instance-specific and thus can be smaller and faster than previous object-aware approaches, while still leveraging category-specific priors incorporated via meta-learned initialization. Our model builds a panoptic radiance field representation of any scene from just color images. We use off-the-shelf algorithms to predict camera poses, object tracks, and 2D image semantic segmentations. Then we jointly optimize the MLP weights and bounding box parameters using analysis-by-synthesis with self-supervision from color images and pseudo-supervision from predicted semantic segmentations. During experiments with real-world dynamic scenes, we find that our model can be used effectively for several tasks like novel view synthesis, 2D panoptic segmentation, 3D scene editing, and multiview depth prediction.

==> [CVPR22] Panoptic Neural Fields/figures/2d_qualitative_comparison.tex <==
\begin{figure}
  \centering
   \includegraphics[width=1.0\linewidth]{figures/2d_qualitative_comparison.jpg}
   \caption{Comparison of semantic segmentation output from Panoptic-DeepLab~\cite{Cheng20cvpr_Panoptic} on ground-truth RGB image, SemanticNeRF~\cite{Zhi21iccv_SemanticNeRF}, and the semantic segmentation rendered from \textbf{our} model from the same view. Segmentation produced by \textbf{our} model is significantly better as highlighted by the red boxes in the figure.}
   \label{fig:ours_vs_deeplab}
   \vspace*{-5mm}
\end{figure}

==> [CVPR22] Panoptic Neural Fields/figures/convergence_shapenet.tex <==
\begin{figure*}[htpb]
\centering
  \includegraphics[width=1.0\linewidth]{figures/convergence_shapenet.jpg}
\caption{Comparison of rendered views with different initialization methods on ShapeNet dataset. \textbf{Top row:} Standard xavier (glorot)~\cite{glorot2010understanding} initialization. \textbf{Bottom row:} Learned initialization via federated averaging. In both cases models were \textbf{only} optimized for two full epochs after the respective initialization. All models were trained on at-least 50 views. See \cref{fig:sparse_views_shapenet} for analysis with sparse views.}
\label{fig:convergence_shapenet}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/fed_avg_illustration.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=1.0\linewidth]{figures/fed_avg_illustration_figure.pdf}
\caption{Category specific learned initialization with federated averaging. \textbf{Upper:} Rather than random initialization of MLP weights, we use meta-learning implemented using FedAvg~\cite{mcmahan2017fedavg,jiang2019improving} to find a good category specific initialization. This allows improves generalization and convergence behavior. \textbf{Lower:} We visualize the learned initialization model for the car class with increasing outer loops of the federated averaging algorithm.}
\label{fig:fed_avg}
\end{figure}

==> [CVPR22] Panoptic Neural Fields/figures/init_illustration.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/init_illustration.jpg}
\caption{This figure illustrates different initialization schemes of instance-specific MLP weights for ``things'' in the car category.}
\label{fig:init_illustration}
\end{figure}

==> [CVPR22] Panoptic Neural Fields/figures/kitti_scene_editing.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/kittti_scene_editing.jpg}
   \caption{Scene editing results. The left column shows rendered color images along  novel viewpoints of our panoptic neural field representations learned on various scenes. Rendered color images from the same view but with edited scene representation are shown in right column. In the first two rows, new objects are introduced to the scene. The third and fourth row shows \textit{cloning} results wherein all \thing MLP weights are duplicated to that of a single object in the scene. The last row shows manipulation of 3D pose of the objects.}
   \label{fig:kitti_scene_editing}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/nvs_kitti360_results.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/nvs_kitti360_results.jpg}
   \caption{Rendered novel views (semantic segmentation and depth) from our Panoptic Neural Field models trained on KITTI-360~\cite{kitti360} scenes. Only the forward facing cameras (captured at $\approx$5Hz) are used for these results. Note that even thin structures like lamp poles and sign-posts are accurately reconstructed and segmented.}
   \label{fig:nvs_kitti360_results}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/nvs_kitti_results.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/nvs_kitti_results.jpg}
   \caption{Rendered novel views (semantic segmentation and depth) from our Panoptic Neural Field models trained on KITTI~\cite{Geiger12cvpr_KITTI} scenes. Only the forward facing cameras (captured at $\approx$ 10Hz) are used for these results. Note that several of the scenes have moving cars but are still accurately reconstructed and segmented.}
   \label{fig:nvs_kitti_results}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/object_prior_architecture.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/object_prior_architecture_landscape.pdf}
\caption{Our framework uses instance-specific fully weight encoded functions to represent each object (left), in comparison to a traditional approach of using one shared MLP with instance-specific latent codes (right). Instance-specific MLPs can be smaller, since they just need to have enough capacity to express a single object instance, as compared to a shared MLP. On scenes with multiple objects our approach can be significantly faster.
% On scenes with multiple objects, even though both approaches have linear complexity in the number of objects, our approach can be significantly faster.
}
\label{fig:instance_specific_neural_function}
\end{figure}

==> [CVPR22] Panoptic Neural Fields/figures/overview.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.935\linewidth]{figures/system_overview_v2.pdf}
\vspace{-0.8em}
\caption{
    Overview of \textit{Panoptic Neural Feld (PNF)} representation being learned from input color images. The background \textit{stuff} is represented by an MLP that produces RGB, density, and semantic logits, while each object is represented by a dynamic track and a smaller individual MLP. Once trained the representation can be used for several tasks by simple volume rendering.
}
\label{fig:system_overview}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/panoptic_3d_reconstruction.tex <==
\begin{figure*}
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{\todo{3D reconstruction and panoptic segmentation.}}
   \label{fig:panoptic_3d_reconstruction}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/renders_2d_gt_boxes.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/renders_2d_gt_boxes.jpg}
  \vspace*{-6mm}
   \caption{Rendered color, depth, instance segmentation, and semantic segmentation images of our models representing dynamic KITTI scenes with various object categories. These results used KITTI \textbf{provided} object tracks. Note that our instance specific object MLPs can also reconstruct novel object categories  like \textit{truck} and ~\textit{bus}.}
   \label{fig:renders_2d_gt_boxes}
   \vspace*{-4mm}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/renders_2d_predicted_boxes.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/renders_2d_predicted_boxes.jpg}
  \vspace*{-6mm}
   \caption{Images of color, depth, instance segmentation, and semantic segmentation rendered on dynamic KITTI scenes from our model trained \textbf{only} from RGB images.}
   \label{fig:renders_2d_predicted_boxes}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/scene_decomp_comp.tex <==
\begin{figure*}
  \centering
%   \includegraphics[width=0.98\linewidth]{figures/NSGvsOurs3x3_touched.jpg}
   \includegraphics[width=1.0\linewidth]{figures/NSGvsOurs-Zoom3.jpg}
   \vspace*{-6mm}
   \caption{Scene decomposition comparison.  Top row: reference views. Middle and Bottom: renderings of objects (without background stuff) of NSG~\cite{nsg21cvpr} and PNF (ours) model respectively. Note that the traffic sign-posts in front of the cars are entangled with the rendered cars in NSG, but not in our results. Also the windows of the bus are correctly reconstructed as translucent by our model.}
   \label{fig:scene_decomp_comp}
   \vspace*{-2mm}
\end{figure*}
% https://docs.google.com/drawings/d/1ldIRdWXsf_iuPshFejCqTXUEkpLECXFfCf0dj_hbfzY/edit?usp=sharing&resourcekey=0-_mWN8XvFSILnX1Moks1OAA

==> [CVPR22] Panoptic Neural Fields/figures/scene_edit.tex <==
\begin{figure}
    \includegraphics[width=1.0\linewidth]{figures/scene_editing.jpg}
   \vspace*{-6mm}
   \caption{Scene editing. We manipulate input ground truth images from KITTI Virtual~\cite{Gaidon16cvpr_virtual_kitti} (top) by cloning all cars to be the same (lower left) or changing their orientations (lower right).}
   \label{fig:scene_edit}
   \vspace*{-2mm}
\end{figure}

==> [CVPR22] Panoptic Neural Fields/figures/sparse_views_shapenet.tex <==
\begin{figure*}[htpb]
\centering
  \includegraphics[width=1.0\linewidth]{figures/sparse_views_shapenet.jpg}
\caption{Comparison of the effect of initialization methods on training \thing models on ShapeNet dataset with \textbf{very sparse} input views. We demonstrate using 1 or 3 image views as input to the model. The input views are shown left. Rendered views of the model when using the standard xavier (glorot)~\cite{glorot2010understanding} initialization are shown in the middle columns. Rendered views with our proposed learned initialization are shown in the right columns. Even with just one image input, our model can reconstruct the cars pretty well.}
\label{fig:sparse_views_shapenet}
\end{figure*}

==> [CVPR22] Panoptic Neural Fields/figures/teaser.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
\centering
\captionsetup{type=figure}
\includegraphics[width=0.98\linewidth]{figures/teaser_pnf.pdf}
\captionof{figure}{
\textit{Panoptic Neural Fields (PNF)} is an object-aware neural scene representation that decomposes a dynamic 3D scene into a set of objects (\things) and background (\stuff), each represented by a separate MLP based neural function. Our model predicts a panoptic-radiance field that represents the color, density, instance, and category label of any 3D point at any given time. The model is trained from RGB images alone and can describe dynamic challenging 3D scenes as shown above.}
%The representation can be employed in a variety of scene understanding tasks, including 3D panoptic segmentation and controllable scene editing.


%Unlike any previous neural representation, PanopticNeRF describes panoptic semantics, handles dynamic scenes, and can be constructed from RGB images alone.
%\textit{\PanopticNerf} represents each object instance as a 3D neural radiance field whose pose changes over time. The static portion of the scene is represented by an additional neural function that predicts the radiance and semantic label for any 3D point in space. Together, these fields represent the density, color, semantic, and instance label of any 3D point at any given time.
%The panoptic-radiance field representation is trained only with self-supervision by minimizing the difference between rendered vs. observed images for both color and semantic segmentation images. 
%The representation can be employed in a variety of scene understanding tasks, including 3D panoptic segmentation and controllable scene editing.
% 
\label{fig:teaser}
\end{center}%
}]

==> [CVPR22] Panoptic Neural Fields/sections/0_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
We present Panoptic Neural Fields (PNF), an object-aware neural scene representation that decomposes a scene into a set of objects (things) and background (stuff).  Each object is represented by an oriented 3D bounding box and a multi-layer perceptron (MLP) that takes position, direction, and time and outputs density and radiance.  The background stuff is represented by a similar MLP that additionally outputs semantic labels. Each object MLPs are instance-specific and thus can be smaller and faster than previous object-aware approaches, while still leveraging category-specific priors incorporated via meta-learned initialization. Our model builds a panoptic radiance field representation of any scene from just color images. We use off-the-shelf algorithms to predict camera poses, object tracks, and 2D image semantic segmentations. Then we jointly optimize the MLP weights and bounding box parameters using analysis-by-synthesis with self-supervision from color images and pseudo-supervision from predicted semantic segmentations. During experiments with real-world dynamic scenes, we find that our model can be used effectively for several tasks like novel view synthesis, 2D panoptic segmentation, 3D scene editing, and multiview depth prediction.
\end{abstract}
\vspace{-0.2in}

==> [CVPR22] Panoptic Neural Fields/sections/1_new_intro.tex <==
\section{Introduction}
\label{sec:introduction}

% \subsection{Problem}
% The ability to understand the content within an image is an essential task in computer vision, and over time we have witnessed a rapid increase in task complexity.
% Over a short period of time, we have progressed from the task of identifying the overall presence of objects within an image~(i.e.~classification~\cite{simonyan2014very, krizhevsky2012imagenet} and object detection~\cite{he2018mask,girshick2015fast}), to fine grained pixel-by-pixel classification~(i.e.~semantic segmentation~\cite{long2015fully,ronneberger2015unet}), and to the ability to differentiate between object instances of the same class~(i.e.~panoptic segmentation~\cite{kirillov2019panoptic, cheng2020panoptic, mohan2021efficientps}).

% Another degree in complexity is introduced by shifting from image to \textit{scene} understanding tasks, where collections of images, potentially in video form, of a consistent scene are provided as input.
% While one could attempt to simply adapt image methods to videos~\cite{trackformer,videopanoptic,choy20194d}, we are specifically interested in problems where these images are observations of the \textit{same} underlying dynamic 3D scene.
% In other words, we expect the images to be explained as the \textit{composition} of a static background with a collection of moving objects, and observed from a moving camera.

% Full 3D scene understanding is important in perception systems for autonomous driving \cite{janai2020computer}, semantic mapping \cite{xia2020survey}, and many other applications involving navigation or operation in the physical world \cite{crespo2020semantic}.
% We are particularly interested in the case where scenes are observed from images captured from car-mounted cameras. Given a sequence of RGB images, our goal is to infer: 1) a 3D reconstruction of the observed geometry, 2) a radiance field of the scene, 3) a decomposition of the scene into potentially dynamic things (e.g., cars) and background stuff (e.g., grass), 4) a category and instance label for every 3D point, as illustrated in \Figure{teaser}.

% \leo{to address frank's concern there can be a paragraph here on how we ``operationalize'' or demonstrate this scene understanding by a number of synthesis tasks, including: 1) the generation of views or depth maps from new camera poses, 2) the inference of 3D-consistent instance or semantic segmentation of these views, and 3) the ability to move and reposition objects in our representation.}
%---------------------------------------------------
% \subsection{Gap}

% Traditional methods for 3D scene understanding require 3D geometry and camera poses~\cite{Wang18cvpr_SGPN, Hou19cvpr_3D-SIS, Lahoud19iccv_MTML, Yang19neurips_BoNet, Yi19cvpr_GSPN, Engelmann20cvpr_3D-MPA, Han20cvpr_OccuSeg, Jiang20cvpr_PointGroup, Nie21cvpr_RfD-Net, Chen21iccv_HAIS} to assign category and instance labels to the input data.  Other methods use SLAM-based pipelines~\cite{SalasMoreno13icra_slam, Narita19iros_Panopticfusion, Rosinol20icra_Kimera, Rosinol20rss_dynamicSceneGraphs} or convolutional networks \cite{Murez20eccv_atlas} to simultaneously predict 3D geometry and semantics.   However, they work only on static scenes, require explicit 3D semantic supervision, and/or rely upon RGB-D inputs. 

% We build upon neural radiance fields (NeRFs) ~\cite{Mildenhall20eccv_nerf}, which represent a scene using a multi-layer perceptron (MLP) that maps positions and directions to densities and radiances.
% Some recent work augments NeRF to infer semantics \cite{Zhi21iccv_SemanticNeRF}, adding an extra head to predict semantic logits for any 3D position along with the usual density/color.
% Other recent work decomposes a scene into a set of NeRFs associated with foreground objects separated from the background \cite{Guo20arxiv_OSF, Yang21iccv_ObjectNeRF, nsg21cvpr}.  However, these systems have several limitations in the context of our goals: 1) they do not produce panoptic segmentations, 2) they learn from scratch for every scene; and 3) they share MLPs for multiple objects, which limits their ability to reproduce specific instances.

% We address these issues by proposing Panoptic Neural Fields (PNF), an object-aware neural scene representation that explicitly decomposes a scene into a set of objects  (\textit{things}), each represented by a \emph{separate} MLP to evaluate the radiance field within the local domain of a potentially moving and semantically labeled 3D bounding box, plus another MLP representing the semantic-radiance field of the background (\textit{stuff}).  Importantly, each object instance is represented by a \emph{separate} MLP that is initialized with a category-specific prior using meta-learning.  This makes it possible to represent instance-specific details with smaller MLPs, which speeds inference in scenes with many objects.
% Together with the background stuff MLP, which includes a semantic head, the object MLPs jointly define a panoptic-radiance field that describes the density, color, category, and instance label of any 3D point at any time.

The ability to understand the content within an image is an essential task in computer vision, and over time we have witnessed a rapid increase in task complexity. Over a short period of time, we have progressed from the task of identifying the overall presence of objects within an image~(i.e.~classification~\cite{krizhevsky2012imagenet} and object detection~\cite{He17iccv_MaskRCNN,girshick2015fast}), to fine grained pixel-by-pixel classification~(i.e.~semantic segmentation~\cite{long2015fully,ronneberger2015u}), and to the ability to differentiate between object instances of the same class (\ie panoptic segmentation~\cite{kirillov2019panoptic,Cheng20cvpr_Panoptic}).

However image level representations described above have limited applications. Instead we are interested in full 3D scene understanding which is  important for autonomous driving \cite{janai2020computer}, semantic mapping \cite{xia2020survey}, and many other applications involving navigation or operation in the physical world \cite{crespo2020semantic}. Given a sequence of RGB images, our goal is to infer: 1) a 3D reconstruction of the observed geometry, 2) a radiance field of the scene, 3) a decomposition of the scene into potentially dynamic things (e.g., cars) and background stuff (e.g., grass), 4) a category and instance label for every 3D point, as illustrated in \Figure{teaser}.

In recent years, neural 3D scene representations like NeRF~\cite{Mildenhall20eccv_nerf} have made significant advancements~\cite{tewari2021advances,xie2021neural}. NeRF represents a scene using a multi-layer perceptron (MLP) that maps positions and directions to densities and radiances which can then be used to synthesize an image from a novel view. However NeRF lacks semantic understanding and is also not object aware. In this work we explore neural scene representations for semantic 3D scene understanding tasks beyond the usual view synthesis task.

Some recent work augments NeRF to infer semantics \cite{Zhi21iccv_SemanticNeRF}, adding an extra head to predict semantic logits for any 3D position along with the usual density/color.
Other recent work decomposes a scene into a set of NeRFs associated with foreground objects separated from the background \cite{Guo20arxiv_OSF, Yang21iccv_ObjectNeRF, nsg21cvpr}.  However, these systems have several limitations in the context of our goals: 1) they do not produce panoptic segmentations, 2) they learn from scratch for every scene; and 3) they share MLPs for multiple objects, which limits their ability to reproduce specific instances.

We address these issues in our proposed Panoptic Neural Fields (PNF), an object-aware neural scene representation that explicitly decomposes a scene into a set of objects (\textit{things}) and amorphous \textit{stuff} background. Each object instance is represented by a \emph{separate} MLP to evaluate the radiance field within the local domain of a potentially moving and semantically labeled 3D bounding box. The semantic-radiance field of the \textit{stuff} background is also represented by a MLP which includes an additional semantic head. Together the \textit{stuff} and \textit{things} MLPs jointly define a panoptic-radiance field that describes the density, color, category, and instance label of any 3D point over time.

Our object aware representation makes it possible to describe scenes with multiple moving objects and also paves the way to incorporate constraints that objects of the same category have similar shape and appearance. Previous object-aware frameworks \cite{nsg21cvpr, Yang21iccv_ObjectNeRF} used a shared MLP with instance-specific latent codes to incorporate this prior. In our model, each object instance is represented by a \emph{separate} MLP that is initialized with a category-specific prior using meta-learning.  The separation of learning of object category priors via meta-learning makes it possible to represent instance-specific details with smaller MLPs, which speeds inference in scenes with many objects.

% \subsection{Implementation}

%\subsubsection{Training/Inference}
Given a collection of images captured from a scene, we employ off-the-shelf algorithms to predict camera parameters~\cite{MurArtal15tro_OrbSLAM} and 2D semantic segmentations~\cite{Cheng20cvpr_Panoptic} for all images, plus a set of 3D object detections with 3D oriented bounding boxes and category labels~\cite{Park21iccv_DD3D}. We initialize the weights of the MLPs for our panoptic neural field model either with object category-specific meta-learned initialization or simple biased initialization of density activation layers.  We then jointly optimize the bounding box and MLP parameters to minimize \textit{analysis-by-synthesis} style losses that measure differences in color and semantic images synthesized with volumetric rendering (as in NeRF \cite{Mildenhall20eccv_nerf}). Thus, our approach provides an unified framework for optimizing 3D shape, appearance, semantics, and object poses all from a set of color images.

%---------------------------------------------------
% \subsection{Evaluation}

We evaluate our method on several scene understanding and synthesis tasks using experiments on the KITTI\cite{Geiger12cvpr_KITTI} and KITTI-360~\cite{kitti360} dataset, including 3D panoptic reconstruction, and scene editing.  The output panoptic-radiance field can also be used to synthesize 2D image-level outputs like semantic segmentation, panoptic segmentation, depth images, and colored images of both observed and novel views.
We demonstrate the utility of the proposed method for these scene understanding tasks, as well as for novel-view synthesis method with movable scene components.

%We also evaluate two approaches for initializing instance-specific MLPs, one based on category specific meta-learning and another based on simple bias initialization of the activation functions.

%---------------------------------------------------
% \subsection{Contributions}

Our contributions can be summarized as follows:
\begin{itemize}
\setlength\itemsep{-.3em}
\item We propose, to the best of our knowledge, the first method that can derive a panoptic-radiance field of complex dynamic 3D scenes from images alone.
\item Our single unified model achieves state-of-the-art quality across multiple tasks and benchmarks on KITTI and KITTI-360 datasets.
\item We incorporate object shape and appearance priors via category-specific meta-learned initialization. This allows our object MLPs to be much smaller and faster than previous object-aware representations.
\item We jointly optimize all (\textit{stuff} and \textit{things}) neural fields and object poses, allowing our method to cope with noisy object poses and image segmentations.
\end{itemize}



==> [CVPR22] Panoptic Neural Fields/sections/2_related.tex <==
\section{Related Work}
\label{sec:related_works}

The most relevant related work is summarized in Table~\ref{tab:related_work} and can be broadly divided into three categories: (1) Learning based single image 3D semantic and/or instance segmentation, (2) Multi-view 3D reconstruction and segmentation methods, and (3) Neural fields.

\textbf{Single image reconstruction and segmentation.}
3D-RCNN~\cite{3drcnn} and Mesh-RCNN~\cite{Gkioxari19iccv_MeshRCNN} takes as input a single RGB image and predicts 3D mesh and pose of object instances in the image. Total3DUnderstanding~\cite{Nie20cvpr_Total3D} combines layout estimation, 3D object detection, and object mesh generation. More recently~\cite{Dahnert21neurips_Panoptic3D} showed 3D panoptic reconstruction and segmentation from a single RGB image.

\input{tables/related_work}

\textbf{Multi-view reconstruction and segmentation:} Incorporating semantics into SLAM and SfM systems has a long history~\cite{hane2013joint,kundu2014joint,blaha2016large,SalasMoreno13icra_slam}.
More recently, PanopticFusion~\cite{Narita19iros_Panopticfusion} is an incremental, online mapping approach that fuses a sequence of RGB-D images into a consistent panoptic segmentation.
ATLAS \cite{Murez20eccv_atlas} reconstructs and labels the 3D geometry from \textit{multiple} posed RGB images. However, ATLAS produces only semantic segmentations (without instances). Both PanopticFusion and ATLAS works only for static scenes, requires 3D supervision, and relies upon convolutions on a discrete voxel grid, which limits its resolution. Kimera~\cite{Rosinol20icra_Kimera} takes a stereo sequence and does online reconstruction, meshing, and semantic labeling of the mesh using \textit{ ground-truth labels}, as a proxy for any 2D segmentation method.
Dynamic Scene Graphs~\cite{Rosinol20rss_dynamicSceneGraphs} expands on that by inferring object instances, even dynamic ones in case of people.
Both methods, though representing impressive systems, were only demonstrated in simulation and rely on ground truth semantic labels.

\textbf{Neural radiance fields (NeRFs).}
This work builds upon NeRF \cite{Mildenhall20eccv_nerf}, which represents a scene using a multi-layer perceptron (MLP) that maps positions and directions to densities and radiances.
From that representation, novel views can be synthesized using volumetric rendering and compared to input views in a self-supervised optimization procedure to infer MLP weights for an observed scene.
However, NeRF only works for static scenes and trains for hours (from scratch) for every set of input views.

\textbf{NeRFs with semantics.} 
Recent work has considered using neural representations to infer semantics \cite{Zhi21iccv_SemanticNeRF}.  In particular, SemanticNeRF \cite{Zhi21iccv_SemanticNeRF} adds an extra head to NeRF to predict semantic labels for any 3D position along with the usual density and color. Concurrent to our work ~\cite{fu2022panoptic} also demonstrated neural panoptic fusion from multiple views. However both of these work are not object aware and cannot handle dynamic scenes.

\textbf{NeRFs with dynamics} disentangle a scene into a canonical volume and its time-varying deformation, represented by a second MLP.
This approach has been applied for deforming faces \cite{Gao20arxiv_pNeRF, Gafni21cvpr_DNRF, Raj21cvpr_ANR}, moving human bodies \cite{Weng20arxiv_vid2actor, Peng21cvpr_NeuralBody, Su21arxiv_A-NeRF}, and objects \cite{Du21iccv_NeRFlow, Li21cvpr_nsff, Park21iccv_nerfies, Pumarola21cvpr_D_NeRF,Xian20cvpr_stnif}.
In contrast, we consider dynamic scenes that contain many moving objects.

\textbf{NeRFs with object decompositions}~\cite{Guo20arxiv_OSF, Yang21iccv_ObjectNeRF, nsg21cvpr} decompose a scene into a set of NeRFs associated with foreground objects separated from the background.
ObjectNeRF~\cite{Yang21iccv_ObjectNeRF} 
% separates the NeRF architecture into scene and object branches, and 
uses the object branch to render rays with masked areas for foreground objects conditioned on a latent code.
Similarly, Neural Scene Graphs (NSGs)~\cite{nsg21cvpr} 
% explicitly separates foreground objects from background, 
uses a separate conditional NeRF for each object category, and a multiplane neural representation for the background.
% Since the NeRFs for foreground objects operate in a local coordinate system, the NSG approach disentangles the object motion from the object and background radiance fields and thus can handle dynamic scenes.
However, these systems have several limitations in the context of our goals: 1) they do not produce panoptic segmentations, 2) they learn from scratch for every scene; and 3) they share NeRFs for multiple objects (which limits the ability to reproduce specific discrete instances).
% All of these issues are addressed in this paper.

\textbf{Conditional NeRFs} infer latent codes as pioneered in GRAF~\cite{Schwarz20neurips_graf}, piGAN~\cite{Chan21cvpr_piGAN}, and PixelNeRF~\cite{Yu21cvpr_pixelNeRF}, as well as the recent CodeNeRF~\cite{Jang21iccv_CodeNeRF}, which also optimizes over object poses. All these works incorporate category-specific priors by sharing MLP weights across object instances, combined with instance specific codes. We instead use instance-specific MLPs for representing each object, which allows each MLP to be smaller, resulting in faster inference speed on scenes with multiple objects. Object appearance and shape priors are incorporated via category-specific meta-learned initialization~\cite{Tancik21cvpr_meta,finn2017maml,nichol2018reptile,jiang2019improving} of the MLP weights.

\iffalse

\section{Comparison to Closely Related Work}

In this section, we contrast our approach and results to those of the most closely related previous work, followed by a discussion of limitations.

Compared to ~\cite{nsg21cvpr}, our model also predicts and reasons about semantics of the scene. Our model also optimizes the object bounding boxes, and is thus robust to noisy bounding boxes predictions of off-the-shelf trackers. Even without the additional supervision from 2D semantic labels, our model achieves better fidelity (measured as PSNR) in reconstructing dynamic scenes and novel compositions. We show improved reconstruction and image quality compared to ~\cite{nsg21cvpr} with significantly smaller (1/10th FLOPs) MLPs per object. Unlike ~\cite{nsg21cvpr}, which uses multi-planes sampling for background model, and for object nodes, restricts the point sampling to those inside the object bounding boxes, we have a simpler and single point sampling strategy (same as \cite{Mildenhall20eccv_nerf}). This also helps with optimizing object bounding boxes, as point samples are not restricted to inside of the current estimate of the object boxes.

Unlike, ObjectNeRF~\cite{Yang21iccv_ObjectNeRF}, our model can represent dynamic scenes. Also our proposed framework is a simpler single stage pipeline, that joint optimizes all the things and stuff NeRFs.

Unlike all previous object centric approaches~\cite{Yang21iccv_ObjectNeRF, nsg21cvpr, Jang21iccv_CodeNeRF}, we take a different architecture to incorporate category-specific object priors. Instead of relying on latent code along with a large category specific MLP, our framework relies on smaller instance specific MLPs with category specific learned initialization using meta-learning. We show improved reconstruction and image quality compared to~\cite{nsg21cvpr} with significantly faster and smaller (1/10th FLOPs) MLP per object during inference.

Unlike SemanticNeRF~\cite{Zhi21iccv_SemanticNeRF}, our model also reasons about object instances, and works for dynamic scenes.

\fi

==> [CVPR22] Panoptic Neural Fields/sections/3_method.tex <==

\newcommand{\image}{\mathcal{C}}
\newcommand{\C}{C} %< color
\newcommand{\gt}{\text{gt}} %< ground truth
\newcommand{\params}{\boldsymbol{\theta}}
\newcommand{\near}{{t_n}}
\newcommand{\far}{{t_f}}
\newcommand{\radiance}{\mathbf{c}}
\newcommand{\sky}{\text{sky}}
\newcommand{\ray}{\mathbf{r}}
\newcommand{\origin}{\mathbf{o}}
\newcommand{\dir}{\mathbf{d}}
\newcommand{\gdir}{\gamma(\dir)}
\newcommand{\density}{\boldsymbol{\sigma}}
\newcommand{\feature}{\mathbf{z}}
\newcommand{\definedAs}{\coloneqq}
\newcommand{\track}{\mathbf{T}}
\newcommand{\tracks}{\track_{\iThing,\iImage}}
\newcommand{\iThing}{k}
\newcommand{\nThings}{K}
\newcommand{\instance}{\mathbf{i}}
\newcommand{\instanceMap}{\mathcal{I}}
\newcommand{\iImage}{i}
\newcommand{\nImages}{I}
\newcommand{\given}{\,|\,}
\newcommand{\depth}{\mathcal{D}}
\newcommand{\point}{\mathbf{x}}
\newcommand{\gpoint}{\gamma(\point)}
\newcommand{\timestamp}{\mathrm{t}}
\newcommand{\semantic}{\mathbf{s}}
\newcommand{\nClasses}{C}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\rotation}{\mathbf{R}}
\newcommand{\translation}{\mathbf{t}}
\newcommand{\size}{\mathbf{s}}
\newcommand{\scale}{\mathbf{s}}

\input{figures/overview}
\section{Method}
\label{sec:method}

This section introduces the panoptic neural field representation and our computational pipeline (Figure~\ref{fig:system_overview}). In ~\cref{sec:scene_rep} we describe the representation itself, which stores a panoptic-radiance field that can be used to query the color, density, semantic and instance labels at any 3D point at any time.  In~\cref{sec:rendering}, we describe how this panoptic-radiance field can be rendered using NeRF-style volume rendering by \textit{over} compositing along sampling of points along rays. In~\cref{sec:model_train} we explain how the model is trained in analysis-by-synthesis style by comparing the rendered color and semantic segmentation with observed 2D color and predicted 2D semantic labels.

A key difference between our framework and previous object-aware frameworks \cite{nsg21cvpr, Yang21iccv_ObjectNeRF} is how we train and represent \things. As illustrated in ~\cref{fig:instance_specific_neural_function}, our framework uses instance-specific fully weight encoded functions to represent each object, in comparison to the traditional approach of using a shared MLP with instance-specific latent codes. This design choice is driven by several factors. First, since the MLP only needs to represent a single object instance, we can have a smaller MLP compared to shared MLPs, resulting in faster inference speed on scenes with multiple objects. Second, this allows the object MLP to use its full capacity to describe and overfit to a specific novel object instance, which may not be possible~\cite{davies2020overfitsdf} with latent encoding. Third, it is simpler and does not require any change to the core NeRF model architecture. Object-level priors can also be incorporated to our instance-specific models using meta-learning based initialization (See \cref{sec:model_init}). 


\subsection{Scene Representation}
\label{sec:scene_rep}

The core of our framework is the panoptic-radiance field representation. This representation accepts input queries consisting of a point position $ \point \in \mathbb{R}^3$, view direction $\dir \in \mathbb{R}^3$, and time $\timestamp \in \mathbb{R}$. The outputs of a query are color, density, a semantic label, and an instance label. This field is the composition of multiple distinct neural functions. There are separate fields for each 3D object (\things), and another, larger field for the background (\stuff). The field associated with one object is defined inside a mobile 3D oriented bounding box. The background is represented by another neural function defined inside a larger scene bounding box. It encodes density, appearance, and semantic labels.

\textbf{Things:}
Foreground objects in our representation are represented by a neural function inside a dynamic bounding box. To instantiate the set of object tracks in a scene, we first run an RGB-only 3D object detector~\cite{Park21iccv_DD3D} and tracker~\cite{pc3t}. This provides a bounding box track $T_{k}$ and semantic class for each recognized object instance $k$. The track is parameterized by a sequence of transformation matrices, one at each of at a set of discrete timestamps. For each timestamp, we create a rotation matrix $\rotation \in \real^{3 \times 3}$ and a translation vector $\translation \in \real^3$. There is also a box extent $\size \in \real^3$ along each axis that is time-invariant.  To determine the coordinate frame of an object at an arbitrary real-valued timestamp, we interpolate the discrete track steps. 

For each object instance, we instantiate a separate time-invariant MLP with the standard NeRF architecture~\cite{Mildenhall20eccv_nerf}. Its weights are initialized using the techniques described in Section~\ref{sec:model_init}.  To query this MLP, positions and directions are transformed from the world frame to the bounding box frame 
% ($\{-1,1\}^3$ map to the corners of the box) 
defined by the track at the current timestamp.
We optimize all parameters of the MLP and object track $T_{k}$ jointly. Optimizing object track parameters is important as initial boxes (even GT boxes) may be noisy. In order to optimize rotation, we orthogonalize $\rotation$ after each gradient descent step using SVD, which projects it back onto $\mathrm{SO}(3)$.

% Each object is represented by an independent instance specific neural function realized with an MLP.
% Position and direction coordinates are first transformed to the object's local coordinate before querying the object MLP to radiance at those coordinates.  We instantiate one object MLP for each object instance in the scene based on our object tracker~\cite{pc3t}. The 3D object pose and bounding box size estimates from the tracker can be noisy and are thus also optimized by our framework. The tracker also assigns a semantic class label to each track which is used as the semantic label for the entire object instance.
% Thus an object $k$ is completely described by MLP weights $\theta_{k}^{\textit{thing}}$, the object track $T_k$, and its semantic label $s_k$. $T_{k,i}$ denotes the state of the track at time instant of an image $i$. The parameterize the tracks state $T_{k,i}=[\rotation,\translation,\size]$, as ac 3x3 rotation matrix , a bounding box center $\translation \in \real^3$, and and bounding box size $\size \in \real^3$. The 3D pose of an object at any arbitrary time can be obtained using interpolation of $T_{k_i}$ using the known timestamps of each image.


\textbf{Stuff:}
We represent the static background \stuff with a single neural function. In addition to predicting density and color at every 3D point, the \stuff function also learns a semantic label per point. We again use an MLP to represent the learned function. The architecture is similar to NeRF, but with an additional head for semantic logits. This head is direction-invariant to encode the inductive bias that 3D points have multi-view consistent semantic labels. Note that unlike the MLPs for objects, which are bounded, the \stuff MLP must handle the unbounded nature of real world scenes. Therefore for large scenes, we follow~\cite{zhang2020nerf++} and use a separate foreground and background \stuff MLPs.

\textbf{Panoptic-Radiance Field:}
The final panoptic-radiance field at a 3D point is computed from aggregating the contributions of the individual \textit{thing} and \stuff MLPs. For any given output channel (color, density, etc.), our function takes the sum of all contributions from any bounding box hits, defaulting to the \stuff output if there is no intersection. For the color field $\radiance$, this is: 
%
\begin{align}
\radiance(\point \given \params) &= \mathbbm{1}_S(\point)\radiance_{s}(\point \given \params) + \sum_\iThing \radiance_\iThing (\track^{-1}_\iThing \point \given \params)
\end{align}
%
 where $\mathbbm{1}_S$ is 1 if and only if the point intersects no bounding boxes, $\radiance_s$ is the \stuff color field, and $\params$ denote the MLP weights for \stuff and \thing MLPs. For other fields, we simply substitute the radiance $\radiance$ with the density, semantic, or instance function. Object boxes contribute a one-hot semantic logit vector for their class, which handles the merging of \stuff and \textit{thing} semantics.
%  (recall that the \stuff output is suppressed inside an object track).
 Similarly, the instance label function is a vector of length $K$, with one dimension per detected object $k$. Objects contribute a one-hot vector for their instance while the \stuff function's instance output is always zero.

\input{figures/object_prior_architecture}

\subsection{Rendering Panoptic-Radiance Fields}
\label{sec:rendering}

Given the complete panoptic-radiance field representation, a 2D image can be synthesized with volume rendering. This process is described in more detail in NeRF~\cite{Mildenhall20eccv_nerf}. Our image synthesis approach is the similar to NeRF, with the addition of support for extra output channels and dynamic boxes. To render a single ray $\ray = \mathbf{o} + t \mathbf{d}$ we uniformly sample $N=1024$ points $\point$ (with jitter) along the ray and alpha-composite the result of the output channel $\C$ we wish to render (RGB, depth, semantic, instance):
%
\begin{align}
\C(\ray \given \params) \approx \sum_{i=1}^{N} w(t_i)f(\ray(t_i) \given \params).
\label{eq:render}
\end{align}
% = \int_\near^\far w(t)\radiance(\ray(t) \given \params) \, dt
Above, $w(t)$ is the final weight associated with each sample, determined by \textit{over} compositing the opacity values of each sample along the ray. The function $f$ returns the representation value for the channel in question at the query point. For semantics, this is logits, while for instance it is a one-hot encoding of the object instance identifier $k$.

\subsection{Model Losses and training}
\label{sec:model_train}

We jointly optimize all network parameters $\theta$ and object tracks $\track$ to reproduce the observed RGB images and predicted 2D semantic images:
%
\begin{align}
\argmin_{\params,\tracks} \:\:
&\loss{rgb} (\params,\tracks)
+ 
\loss{sem} (\params,\tracks)
\label{eq:optim}
\end{align}
%
At each gradient descent step, we randomly sample mini-batches of rays. Our RGB loss is the mean squared error between the synthesized and ground truth color, summed over sampled rays as in NeRF~\cite{Mildenhall20eccv_nerf}. Our semantic loss is applied at the same pixel locations, and compares the synthesized semantics with the input 2D semantic segmentation prediction~\cite{Cheng20cvpr_Panoptic}. For this loss, we apply a per-pixel softmax-cross entropy function rather than mean squared error.

% Our model is trained using the classical analysis-by-synthesis style supervision. The 3D panoptic-radiance field representation produced by our model is differentiably rendered as described above to produce 2D color and segmentation pixels (synthesis), which are then compared with pixels from observed color and segmentation images to optimize the parameters of our 3D scene representation model (analysis).

% Concretely, we optimize all $k$ object MLP weights $\theta_{k}^{\textit{thing}}$ and object tracks $\tracks$:


% The RGB 

% \begin{equation}
% \loss{rgb}(\params) = \sum_\iImage \expect_{\ray \sim \image_\iImage^\gt}
% ||\C(\ray \given \params) - \C^\gt_\iImage(\ray) ||_2^2.
% \label{eq:nerf}
% \end{equation}

% We incorporate semantic supervision from by minimizing softmax cross-entropy $CE$ with respect to input semantic maps $\S^\gt_\iImage(\ray)$:
% % 
% \begin{align}
% \loss{sem}(\params) &= \sum_\iImage \expect_{\ray \sim \S_\iImage^\gt}
% \left[
% \text{CE}( \S(\ray), \S^\gt_\iImage(\ray) ) 
% \right].
% \label{eq:sem}
% \end{align}

\input{figures/init_illustration}
\input{figures/fed_avg_illustration}

\subsection{Incorporating priors via initialization}
\label{sec:model_init}
One of the core benefits of an object aware approach, is the ability to incorporate inductive bias that objects instances within same category, often have similar 3D shape and appearance. One possible way to incorporate such priors is to have shared MLP weights across all object instances, combined with some instance specific codes. Our framework instead uses separate MLPs for representing each object instance. As illustrated in ~\cref{fig:instance_specific_neural_function}, this allows each MLP to be smaller as it only needs to represent a single object instance, resulting in faster inference speed on scenes with multiple objects. Object shape and appearance priors are instead incorporated via initialization of the MLP weights of the neural functions. We present two approaches (see \cref{fig:init_illustration}) of initializing our model, one based on category specific meta-learning and another based on simple bias initialization of the activation function of the MLPs.

% A core benefit of an object-aware approach is that we can incorporate the inductive bias that object instances of the same semantic category often have similar 3D shape and appearance. One possibility is to share MLP weights across all object instances of a class, combined with instance-specific latent codes (\cref{fig:instance_specific_neural_function}, right). However, these shared MLP needs be large enough to capture details for each object instance. Hence, per-query cost increases rapidly with the number of objects in the scene. In our framework, object appearance and shape priors are instead incorporated via initialization of the MLP weights of the neural functions. We present two approaches of initializing our models, one based on category specific meta-learning and another based on simple bias initialization of the activation function of the MLPs. See \cref{fig:init_illustration} for illustration of these two initialization schemes.


% To address this problem, we use a separate MLP per object instance, and instead incorporate priors through a shared \textit{initialization} (\cref{fig:instance_specific_neural_function}, left). Our approach allows each MLP to be smaller as it only needs to represent a single object instance. This improves inference performance. Furthermore, we are still able to incorporate category specific priors via meta-learning when training data is available. Below we present two approaches for MLP initialization, each of which is useful depending on the experimental context (see \cref{fig:init_illustration}).
% 
\input{figures/renders_2d_predicted_boxes}
\input{figures/renders_2d_gt_boxes}

\textbf{Biased initialization:}
This simple initialization scheme improves convergence behavior and training performance without requiring a large dataset from which to learn a shape prior. In real-world outdoor scenes, most of the \stuff volume is empty space. By contrast, most of the volume inside each \things object bounding box is non-empty. We incorporate this prior directly by biasing the density prediction layer of the MLPs. For the \stuff MLP, we initialize our bias to $-5.0$, whereas for all \thing MLPs, we initialize the final bias layer to $0.1$. 
Furthermore, for all MLPs, we use the \textit{softplus} activation for the fully connected layer predicting the density outputs~\cite{Zheng15ijcnn_softplus}. We have found that this simple injection of prior knowledge via initializing the bias values is quite effective and robust compared to random initialization, since dense content in \stuff can suppress gradients from distant objects.

\textbf{Category specific learned initialization:}
If a large shape collection is available for certain object categories, we can further improve on the bias initialization scheme. In particular, we use meta-learning~\cite{finn2017maml} to capture category-specific shape and appearance priors. This process is illustrated in \cref{fig:fed_avg}. First, we meta-learn category-specific initial weights by pre-training on ShapeNet~\cite{chang2015shapenet}. Then, we use these weights to initialize the \thing MLPs in our model when training on a novel scene.

To meta-learn a category-specific shape prior, we use the \texttt{FedAvg}~\cite{mcmahan2017fedavg} algorithm. This algorithm is known to be equivalent~\cite{jiang2019improving} to REPTILE~\cite{nichol2018reptile} meta-learning, used before for NeRF initialization in \cite{Tancik21cvpr_meta}.  
To do one meta-step of \texttt{FedAvg}, we independently optimize a set of MLPs, each on a separate ShapeNet shape. We then average the model weights across all NeRF models, and start another meta-step. \cref{fig:fed_avg} visualizes the evolution of the learned initialization across several outer loops of \texttt{FedAvg}. In our experiments, we pre-train using the 2D rendered car images~\cite{Sitzmann19neurips_srn} of ShapeNet~\cite{chang2015shapenet} to obtain the learned initialization model. When reconstructing a full scene, we then initialize the MLPs for each car instance track $\track$ to this initialization.

==> [CVPR22] Panoptic Neural Fields/sections/4_experiments.tex <==


\section{Evaluations}\label{sec:evaluation}

We performed a series of experiments to evaluate our model on multiple computer vision tasks, including view synthesis, reconstruction, 2D panoptic segmentation, 2D depth prediction, and scene editing. See the supplemental video for comprehensive visualizations of our results. All experiments used either the KITTI \cite{Geiger12cvpr_KITTI}, Virtual KITTI \cite{Gaidon16cvpr_virtual_kitti, Cabon20arxiv_virtual} or the recent KITTI-360~\cite{kitti360} datasets. These datasets involves difficult forward facing cameras in complex outdoor dynamic scenes. KITTI-360 is the first benchmark that evaluates both the task of synthesising color and appearance images from novel views. Our model outperforms every other method in that leaderboard for both tasks as shown in \cref{tab:kitti360}. Since scenes in KITTI-360 chosen for the tasks are all static, we also evaluate our model on dynamic scenes from the KITTI~\cite{Geiger12cvpr_KITTI} dataset. Rendered views from these dynamic scenes are shown in \cref{fig:renders_2d_predicted_boxes} and \cref{fig:renders_2d_gt_boxes}. Additional results are available in \cref{sec:additional_results}. Below we evaluate our model for each task in more detail.

% ---------

\input{tables/kitti360_nvs50}
\input{tables/quantitative_kitti_nsg}

\textbf{Novel View Synthesis:}
How well a particular representation describes a scene is reflected in the quality of rendered views. As shown in~\cref{tab:kitti360}, color images rendered by our model achieves the best PSNR and is competitive with latest view synthesis models~\cite{Mildenhall20eccv_nerf,Riegler2020ECCV,kopanas2021point,Barron21iccv_Mip_NeRF}. Since the scenes used in KITTI-360~\cite{kitti360} novel view synthesis task are all static, we attribute the improved performance to our model benefiting from separate object-aware MLPs and incorporation of category-level priors. To study the novel view synthesis capabilities of our model on dynamics scenes, we also experiment on several dynamic scenes from KITTI dataset as shown in leftmost columns of \cref{fig:renders_2d_predicted_boxes} and \cref{fig:renders_2d_gt_boxes}. Notice that the rendered color images accurately captures the moving vehicles in the scene. A quantitative analysis of synthesized colored images for dynamic KITTI scenes is available in~\cref{tab:quantitative_kitti_nsg}, wherein we follow the same experimental setup as described in Sec.~5.2 of Ost~\etal~\cite{nsg21cvpr}. As expected, our method significantly outperforms representations like SRN~\cite{Sitzmann19neurips_srn} and NeRF~\cite{Mildenhall20eccv_nerf} which rely on static world assumption. Note that our method also outperforms NSG~\cite{nsg21cvpr} even though our instance specific object MLPs are much smaller ($10\times$ fewer FLOPs) compared to those used in NSG~\cite{nsg21cvpr}. The improvement over NSG also demonstrates the advantage of incorporating category-specific priors derived from meta-learning with images from ShapeNet.

% ---------

\input{tables/segmentation_2d}
\input{figures/2d_qualitative_comparison}

\input{figures/scene_decomp_comp}
\input{figures/scene_edit}

\textbf{Panoptic Segmentation:}
Semantic and instance segmentation of an arbitrary view can be obtained from our model by simple rendering (see \cref{eq:render}) along the desired view. The two right columns of \cref{fig:renders_2d_predicted_boxes} and \cref{fig:renders_2d_gt_boxes} demonstrates the rendered semantic and instance segmentation images from our model. As shown in \cref{tab:kitti360}, our model achieves \textit{state-of-the-art} 74.28 mIoU for the task of novel view semantic segmentation on KITTI-360. One approach of generating segmentation images for any arbitrary view is to first synthesize color image from a desired view using view synthesis methods like ~\cite{Mildenhall20eccv_nerf,Riegler2020ECCV,kopanas2021point,Barron21iccv_Mip_NeRF}; followed by 2D image segmentation~\cite{zhao2017pyramid,Cheng20cvpr_Panoptic}. However as demonstrated in \cref{tab:kitti360}, our unified model significantly outperforms all such two-stage baselines. Moreover the rendered segmentation images from our model are temporally consistent and works for dynamic scenes. We also perform a ablation study of the rendered segmentation images on dynamic scenes from KITTI. Quantitative and qualitative results are shown in \cref{tab:segmentation_2d} and \cref{fig:ours_vs_deeplab} respectively. Our model significantly out performs (+9.2 mIoU) non object-aware models like SemanticNeRF~\cite{Zhi21iccv_SemanticNeRF}, since they cannot model dynamic objects. Our model also improves upon single image state-of-the-art segmentation models~\cite{Cheng20cvpr_Panoptic} by fusing information from multiple views.

\textbf{2D Depth Estimation:} We also demonstrate rendered depth images from our model, obtained by over compositing point depths along rays with opacity values as described in~\cref{eq:render}. Rendered depth images are shown in the second columns of ~\cref{fig:renders_2d_predicted_boxes,fig:renders_2d_gt_boxes}, along with other outputs of the model. Please note the sharp reconstruction of shapes of moving cars on the road. Of course, those cars would be missing or blurred in standard NeRF models. This demonstrates the benefits of our object-aware approach that handles dynamic scenes and instance-specific object MLPs that accurately captures each object instance.

\textbf{Object Decomposition:}
\cref{fig:scene_decomp_comp} shows visualizations of how images from a dynamic KITTI scene are decomposed into MLPs representing different object instances. These images are rendered without the (stuff) background. Compared to NSG~\cite{nsg21cvpr}, our method does a better job of disentangling objects from the (stuff) background. In particular, note that the occluding traffic sign-posts in front of the car are entangled with the rendered cars in NSG, but not in our results. Better object decomposition from our model is also important for the scene editing task discussed below.

% ---------
\textbf{Scene Editing:}
Since our model separates objects from the background and builds a full 3D radiance field for each object, it is possible to edit images using the model by removing objects, adding new objects, and transforming object bounding boxes and poses. \cref{fig:scene_edit} shows few scene editing examples on Virtual KITTI dataset. The top row shows original images, and the bottom row shows edits. In bottom-left, we demonstrate \textit{cloning} of cars by replicating the weights of all object MLPs to a same car. In bottom right of the figure we independently rotate each vehicle object.


% ---------

% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------


==> [CVPR22] Panoptic Neural Fields/sections/5_conclusion.tex <==
\section{Limitations}
\label{sec:limitations}
Like most other NeRF-style methods, our model is compute-intensive and hence currently only suited for offline applications. However, we expect advances in neural rendering \cite{muller2022instant,tewari2021advances} will alleviate some of these speed issues in near future. It also does not incorporate more complex light transport effects, such as shadowing, under object motion.
Our framework optimizes and corrects bounding box poses from  noisy 3D object detection and tracking, but has not been designed to handle other errors such as missing and duplicate detections and incorrect class predictions. 
Finally, our framework does not handle deformable objects and is restricted to scenes with rigid moving objects.
% These limitations, failure cases, and a discussion of potential negative societal impacts are discussed further in the supplemental material.

\section{Conclusion}
\label{sec:conclusion}
This paper presents Panoptic Neural Fields (PNF), an object-aware neural scene representation that decomposes a scene into a set of MLPs associated with object instances (\things) and the background (\stuff). Our model learns a 4D panoptic radiance representation of dynamic scenes from images alone. This representation can be queried to obtain the color, density, instance, and category label of any 3D point over time. Several tasks like scene editing, view synthesis, panoptic segmentation are derived by simply rendering the representation from the desired views. Results of experiments on several KITTI scenes demonstrate state-of-the-art performance for novel view synthesis and panoptic segmentation for challenging outdoor scenes with multiple dynamic objects.

==> [CVPR22] Panoptic Neural Fields/tables/kitti360_nvs50.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lcc}
\hline
Method                                                                  & Semantics mIoU & Appearance PSNR \\ \hline
NeRF~\cite{Mildenhall20eccv_nerf} + PSPNet~\cite{zhao2017pyramid}       & 53.01          & 21.18      \\
FVS~\cite{Riegler2020ECCV} +  PSPNet~\cite{zhao2017pyramid}             & 67.08          & 20.00      \\
PBNR~\cite{kopanas2021point} + PSPNet~\cite{zhao2017pyramid}            & 65.07          & 19.91      \\
Mip-NeRF~\cite{Barron21iccv_Mip_NeRF} + PSPNet~\cite{zhao2017pyramid}   & 51.15          & 21.54      \\
\textbf{Ours}                                                           & \textbf{74.28} & \textbf{21.91} \\ \hline
\end{tabular}
} %< \resizebox
\vspace*{-2mm}
\caption{
% 
Results on novel view color and semantic synthesis tasks on KITTI-360~\cite{kitti360} dataset. Rendered semantic segmentation and color images from our model is the best performing method for both the tasks in KITTI-360 leaderboard.
% 
} % \caption
\label{tab:kitti360}
\end{table}

==> [CVPR22] Panoptic Neural Fields/tables/quantitative_kitti_nsg.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccccc}
\multicolumn{1}{l|}{}          & SRN~\cite{Sitzmann19neurips_srn}   & NeRF~\cite{Mildenhall20eccv_nerf}  & NeRF + time & NSG~\cite{nsg21cvpr}   & Ours           \\ \hline
\multicolumn{1}{l|}{PSNR $\uparrow$}      & 18.83 & 23.34 & 24.18       & 26.66 & \textbf{27.48} \\
\multicolumn{1}{l|}{SSIM $\uparrow$}      & 0.590 & 0.662 & 0.677       & 0.806 & \textbf{0.870}   \\
\end{tabular}
} % \resizebox
\vspace*{-2mm}
\caption{Comparison of image reconstruction quality in dynamic KITTI scenes following the the experiement setup of NSG~\cite{nsg21cvpr}. 
% Our method can better reconstruct color images of the scene as measured with PSNR and SSIM metrics.
} % \caption
\label{tab:quantitative_kitti_nsg}
\vspace*{-4mm}
\end{table}

==> [CVPR22] Panoptic Neural Fields/tables/related_work.tex <==
\definecolor{dark-green}{rgb}{0.0, 0.5, 0.0}
\newcommand{\chg}{\textcolor{dark-green}{\chk}}

\begin{table}[t]
\centering
\small
% "tabular" below auto-generated from Airtable, please do not edit, talk to Frank instead
\begin{tabular}{p{3cm}p{4mm}p{4mm}p{4mm}p{4mm}p{4mm}p{4mm}}
\hline
 Paper                                                     & Sem   & Obj   & Pan   & Dyn   & Opt   &  Syn  \\
\hline
%  SGPN~\cite{Wang18cvpr_SPGN}                               & \chk  & \chk  &       &       &       \\
%  3D-SIS~\cite{Hou19cvpr_3D-SIS}                            & \chk  & \chk  &       &       &       \\
%  MTML~\cite{Lahoud19iccv_MTML}                             & \chk  & \chk  &       &       &       \\
%  3D-BoNet~\cite{Yang19neurips_BoNet}                       & \chk  & \chk  &       &       &       \\
%  GSPN~\cite{Yi19cvpr_GSPN}                                 & \chk  & \chk  &       &       &       \\
%  3D-MPA~\cite{Engelmann20cvpr_3D-MPA}                      & \chk  & \chk  &       &       &       \\
%  OccuSeg~\cite{Han20cvpr_OccuSeg}                          & \chk  & \chk  &       &       &       \\
%  PointGroup~\cite{Jiang20cvpr_PointGroup}                  & \chk  & \chk  &       &       &       \\
%  RfD-Net~\cite{Nie21cvpr_RfD-Net}                          & \chk  & \chk  &       &       &       \\
%  HAIS~\cite{Chen21iccv_HAIS}                               & \chk  & \chk  &       &       &       \\
% \hline
 MeshRCNN~\cite{Gkioxari19iccv_MeshRCNN}                   &       & \chk  &       &       &       &       \\
 Total3D~\cite{Nie20cvpr_Total3D}                          & \chk  & \chk  &       &       &       &       \\
 \hline
 Atlas~\cite{Murez20eccv_atlas}                            & \chk  &       &       &       &       &       \\
SLAM++\cite{SalasMoreno13icra_slam}                      &       & \chk. &       &       &       &       \\
PanopticFusion~\cite{Narita19iros_Panopticfusion}          & \chk  &       & \chk  &       &       &       \\
 Kimera~\cite{Rosinol20icra_Kimera}                        & \chk  &       &       &       &       &       \\
 DynSceneGraphs~\cite{Rosinol20rss_dynamicSceneGraphs} & \chk  & \chk  & \chk  & \chk  & \chk  &       \\
\hline
%  IMAP~\cite{Sucar21iccv_iMAP}                              &       &       &       &       &       &       \\
 SemanticNerF~\cite{Zhi21iccv_SemanticNeRF}                & \chk  &       &       &       &       & \chk \\
 NSG~\cite{nsg21cvpr}                                  &       & \chk  &       & \chk  &       & \chk \\
 ObjectNeRF~\cite{Yang21iccv_ObjectNeRF}                   &       & \chk  &       &       &       & \chk \\
\hline
 PNF (Ours)                                       & \chg  & \chg  & \chg  & \chg  & \chg  & \chg \\
\hline
\end{tabular}
%------------------------------- end generated -----------------------------------------------------
\caption{Comparison to properties of related work.   The check marks indicate which prior methods have the following capabilities:   
``Sem'' = performs semantic segmentation;
``Obj'' = performs object decomposition;
``Pan'' = performs panoptic segmentation;
``Dyn'' = handles dynamic objects; and
``Opt'' = optimizes object bbox parameters.
``Syn'' = allows for novel view synthesis.
}
\label{tab:related_work}
\end{table}

==> [CVPR22] Panoptic Neural Fields/tables/segmentation_2d.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lcc}
\toprule
Method                                    & mIoU            & PQ\\ \midrule
2D Deeplab~\cite{Cheng20cvpr_Panoptic} on ground-truth RGB       & 49.9            & 43.2 \\
2D Deeplab~\cite{Cheng20cvpr_Panoptic} on NeRF rendered RGB      & 32.1            & 24.9 \\
\textbf{Ours} without \thing MLPs ($\approx$\textit{SemanticNeRF})                             & 45.3            & - \\
\textbf{Ours}                             & \textbf{56.5}   & \textbf{45.9} \\ \bottomrule
\end{tabular}
} %< \resizebox
\vspace*{-2mm}
\caption{
Ablation study of the rendered segmentation quality on KITTI. Our model achieves better segmentation in terms of mean IoU, panoptic quality (PQ)~\cite{kirillov2019panoptic}. Also notice that without \thing MLPs, the segmentation quality is significantly worse and misses all dynamic objects. This demonstrates the advantage of our model over non object-aware representations like \textit{SemanticNeRF}~\cite{Zhi21iccv_SemanticNeRF}.
} % \caption
\label{tab:segmentation_2d}
\end{table}

==> figures/panoptic_3d_reconstruction.tex <==
\begin{figure*}
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{\todo{3D reconstruction and panoptic segmentation.}}
   \label{fig:panoptic_3d_reconstruction}
\end{figure*}
